Analogue Quantum Simulation: A Philosophical Prospectus

This paper provides the first systematic philosophical analysis of an increasingly important part of modern scientific practice: analogue quantum simulation. We introduce the distinction between `simulation' and `emulation' as applied in the context of two case studies. Based upon this distinction, and building upon ideas from the recent philosophical literature on scientific understanding, we provide a normative framework to isolate and support the goals of scientists undertaking analogue quantum simulation and emulation. We expect our framework to be useful to both working scientists and philosophers of science interested in cutting-edge scientific practice.

==> commands.tex <==

%%%================================================================
%%%================      new commands      =======================
%%%================================================================

\newcommand\hcancel[2][black]{\setbox0=\hbox{$#2$}%
\rlap{\raisebox{.45\ht0}{\textcolor{#1}{\rule{\wd0}{1pt}}}}#2} 



%
%%% ---------------------- Referencing-------------------------

\newcommand{\tabr}[1]{Table~\ref{#1}}
\newcommand{\eqr}[1]{Eq.~(\ref{#1})}
\newcommand{\fir}[1]{Fig.~\ref{#1}}
\newcommand{\secr}[1]{Sec.~\ref{#1}}
\newcommand{\apr}[1]{App.~\ref{#1}}
\newcommand{\chr}[1]{Ch.~\ref{#1}}

% % Theorem environments
% 
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{protocol}{Protocol}
\newtheorem{conjecture}{Conjecture}
% 
\newtheorem{cor}{Corollary}
\newtheorem*{remark}{Remark}

%%% ---------------------- Custom Colors-------------------------

\definecolor{DarkGray}{gray}{0.25} 
\definecolor{MidGray}{gray}{0.38} 
\definecolor{NeutralGray}{gray}{0.5}
\definecolor{LightGray}{gray}{0.7}
\definecolor{lightGray}{gray}{0.85}
\definecolor{DarkRed}{rgb}{0.7,0,0}
\definecolor{DarkBlue}{rgb}{0,0,0.5}
\definecolor{SteelBlue}{rgb}{0,0.4,0.6}
\definecolor{Orange}{rgb}{0.7,0.5,0}
\definecolor{Violette}{rgb}{0.5,0,0.5}
\definecolor{Sand}{rgb}{0.84,0.8,0.55}
\definecolor{niceblue}{rgb}{0.33,0.5,0.8}
\definecolor{OliveGreen}{RGB}{0,102,102}
\definecolor{NiceGreen}{RGB}{0,153,72}
\definecolor{LightGreen}{RGB}{0,200,72}
\definecolor{newblue}{RGB}{40,210,251}
\definecolor{lightblue}{RGB}{179,231,251}
\definecolor{steelblue}{RGB}{70,130,180}
\definecolor{cred}{RGB}{179,28,28}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\usepackage{tcolorbox}

\tcbset{
    coltitle=black,fonttitle=\bfseries,
    colback=orange!7!white,colframe=gray!25!white,width=0.95\textwidth,valign=center,
    before=\par\bigskip\centering,after=\par
    }


%%% ---------------------- Operators -------------------------
%Use either \DeclareMathOperator or \operatorname http://tex.stackexchange.com/questions/84302/what-is-the-difference-of-mathop-operatorname-and-declaremathoperator

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\rg}{range}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\dist}{d}
\DeclareMathOperator{\spec}{spec}
\DeclareMathOperator{\trunc}{\upharpoonright}

\newcommand{\rmd}{\mathrm{d}}
\DeclareMathOperator{\landauO}{O}
% \newcommand{\trunc}[2]{#1_{\upharpoonright \mathnormal{#2}}} %truncation
\DeclareMathOperator{\cc}{c.c.}
\DeclareMathOperator{\hc}{h.c.}
 
%%% ---------------------- Others-------------------------
\newcommand{\ad}{^\dagger}
\newcommand{\restr}{\upharpoonright}
\DeclareMathOperator{\dunion}{\uplus}%Disjoint union
\DeclareMathOperator{\dUnion}{\biguplus}%Disjoint union
\renewcommand{\complement}{^{c}}
\DeclareMathOperator{\colonequiv}{:\!\Leftrightarrow}

\newcommand{\iprod}[2]{( #1, #2)}
\newcommand{\Iprod}[2]{\left( #1, #2 \right)}

\newcommand{\set}[1]{\{ #1  \}}
\newcommand{\Set}[1]{\left \{ #1 \right \}}

\newcommand{\dt}[1]{\frac{\partial #1}{\partial t}}



%%% ---------------------- brakets -----------------
%\usepackage{braket}
\renewcommand{\l}{\langle}
\renewcommand{\r}{\rangle}
\newcommand{\Ket}[1]{\left|{#1}\right\rangle}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\Bra}[1]{\left\langle{#1}\right|}
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\braket}[2]{\left\langle{#1}\middle|{#2}\right\rangle}
\newcommand{\ketn}[1]{| #1 \rangle}
\newcommand{\bran}[1]{\langle #1 |}
\newcommand{\braketn}[2]{\langle #1 \middle| #2 \rangle}
\newcommand{\ketbra}[2]{\ket{#1} \!\! \bra{#2}}
\newcommand{\ketbran}[2]{\ketn{#1} \! \bran{#2}}
\newcommand{\proj}[1]{\ket{#1}\bra{#1}}
\newcommand{\Proj}[1]{\Ket{#1}\Bra{#1}}
\newcommand{\Sandwich}[3]
  {\left\langle  #1 \right| #2 \left| #3 \right\rangle}
  
\newcommand{\sandwich}[3]
  {\langle  #1 | #2 | #3 \rangle}
  
\newcommand{\Av}[1]{\left\langle #1 \right\rangle}
\newcommand{\av}[1]{\langle #1 \rangle}
\newcommand{\avb}[1]{\bigl\langle #1 \bigr\rangle}
\newcommand{\avB}[1]{\Bigl\langle #1 \Bigr\rangle}

%%% ----------------- norms ----------------------
\newcommand{\Norm}[1]{\left\Vert #1\right\Vert}
\newcommand{\norm}[1]{\Vert #1\Vert}
\newcommand{\normt}[1]{\boldsymbol{\vert} #1\boldsymbol{\vert}}
\newcommand{\normone}[1]{\| #1 \|_1}
\newcommand{\norminf}[1]{\| #1 \|_\infty}
\newcommand{\normuinv}[1]{||| #1 |||}
\newcommand{\hnorm}[1]{||| #1 |||}
\newcommand{\normb}[1]{\bigl\| #1 \bigr\|}
\newcommand{\normB}[1]{\Bigl\| #1 \Bigr\|}
\newcommand{\abs}[1]{\lvert #1\rvert}
\newcommand{\Abs}[1]{\left\lvert #1\right\rvert}


%%% ---------------------- Letters-----------------

\newcommand{\ee}{\mathrm{e}}
\newcommand{\ii}{\mathrm{i}}
\newcommand{\dd}{\mathrm{d}}


\newcommand{\GG}{\mathbf{G}}
\newcommand{\LL}{\mathbf{L}}
\newcommand{\VV}{\mathbf{V}}


\newcommand{\qb}{\mathbf{q}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\rb}{\mathbf{r}}
\renewcommand{\sb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}


\newcommand{\jc}{\mathcal{j}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}

\newcommand{\Ab}{\mathbb{A}}
\newcommand{\Cb}{\mathbb{C}}
\newcommand{\Eb}{\mathbb{E}}
\newcommand{\Lb}{\mathbb{L}}
\newcommand{\Nb}{\mathbb{N}}
\newcommand{\Pb}{\mathbb{P}}
\newcommand{\Qb}{\mathbb{Q}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Tb}{\mathbb{T}}
\newcommand{\Zb}{\mathbb{Z}}
\newcommand{\idb}{\mathbb{1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% Specific to this project
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

% Complexity classes
\newcommand{\sat}{\textsf{SAT}}
\newcommand{\qsat}{\textsf{QSAT}}

\newcommand{\p}{\textsf{P}}
\newcommand{\bpp}{\textsf{BPP}}
\newcommand{\np}{\textsf{NP}}
\newcommand{\pH}{\textsf{PH}}

\renewcommand{\sp}{\#\textsf{P}}

\newcommand{\bqp}{\textsf{BQP}}
\newcommand{\qma}{\textsf{QMA}}
\newcommand{\ma}{\textsf{MA}}

%%% -------------------------- Commments ----------------------------

\newcommand\contribution[1]{\emph{\textcolor{gray!40!black}{#1}}}
\newcommand{\ins}[1]{\textcolor{cred}{*** #1 ***}}
\newcommand{\doha}[1]{\textcolor{cyan}{[DoHa: #1]}}


==> tikzdef.tex <==


\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15)
-- cycle;} 
%%% --------------- references -----------------------
\newcommand{\refs}[1]{
%\begin{tikzpicture}[remember picture, overlay]
  \node (refs) at (current page.south west) [anchor = south west, xshift = .5cm]{
    \begin{minipage}{.975\linewidth}
    \tiny
    #1
    \end{minipage}
  };
  \draw (refs.north west) -- ++(.3\linewidth,0);
%\end{tikzpicture}  
}
\newcommand{\Refs}[1]{
	\begin{tikzpicture}[remember picture, overlay]
	\refs{#1}
	\end{tikzpicture}  
}

\newcommand{\bigtikzitem}[1]{
  \begin{tikzpicture}[baseline={([yshift=-0.85ex]current bounding box.center)}]
    \fill[niceblue] (0,0) rectangle (0.5,0.5) node[midway,anchor=center,color=white,overlay] {\footnotesize $#1$};
  \end{tikzpicture}
}

\newcommand{\tikzitem}[1]{ $ \ $
  \begin{tikzpicture}[baseline={([yshift=-.3\baselineskip]current bounding box.west)}]
    \fill[niceblue] (0,0) rectangle (0.3,0.3) node[midway,anchor=center,color=white,overlay] {\footnotesize $#1$};
  \end{tikzpicture}
}

\newcommand{\smalltikzitem}{ $ \ $
  \begin{tikzpicture}[baseline={([yshift=-.25\baselineskip]current bounding box.west)}]
    \fill[niceblue] (0,0) rectangle (0.17,0.17);
  \end{tikzpicture}
}

\newcommand{\tikznode}[1]{%
  \tikz[remember picture,%
	overlay,%
	baseline={([yshift=-.25\baselineskip]current bounding box.west)},%
       ]{
	 \node[minimum height = 1\baselineskip, inner sep = 0] (#1){};% node
	}% tikz
}% newcommand

\newcommand{\graylrarrow}{%
  \tikz[baseline = -.2\baselineskip]
    {\draw [<->, connection edge] (0,0)--++ (1em,0);
  }\hspace{.6ex}%
}

\newcommand{\grayrarrow}{%
  \tikz[baseline = -.2\baselineskip]
    {\draw [->, connection edge] (0,0)--++ (1em,0);
  }\hspace{.6ex}%
}

%%% ---------------- spin chains --------------------
\newcommand{\spinchain}{
    \begin{tikzpicture}[
	  anchor = center, 
	  vertex/.style = {circle,inner sep = 1.1ex},
	  edges/.style = {very thick, line cap = round, gray},
	  ]
      \clip (\nx,0) ++ (-.5,-.5) rectangle (.5,.5);
      %
      \foreach \x in {0,1,...,\nx}
	  \node (v\x) [vertex] at (\x,0){}; 
      %edges
      \foreach \x in {1,2,...,\nx}{
	\pgfmathsetcount{\xm}{\x-1};
	\draw[edges] (v\x) -- (v\the\xm);
      }

      %draw vertices
      \foreach \x in {0,1,...,\nx}{
        \draw[gray] (\x,0) circle (.9ex); %hack for pdf viewers that do not draw ball shading correctly 
        \shade[ball color=VertexCol] (\x,0) circle (.9ex);% node[beschriftung]{\tiny \x,\y}; 
    % 	\node[fill=white] at (\x,\y) {\tiny \x,\y}; % lable coordinates 
      }
    \end{tikzpicture}
}

\newcommand{\hotspinchain}{
       \begin{tikzpicture}[anchor = center,
	  vertex/.style = {circle,inner sep = 1.1ex},
	  edges/.style = {very thick, line cap = round, gray},
	  ]
      \clip (\nx,0) ++ (-.5,-.5) rectangle (.5,.5);
      %
      \foreach \x in {0,1,...,\nx}
	  \node (v\x) [vertex] at (\x,0){}; 
      %bath
      \foreach \x in {1,...,\nx}{
	\pgfmathsetcount{\xm}{\x-1};
	\node [ellipse, fit = (v\the\xm) (v\x), draw, fill = red, inner sep = -.5ex, opacity = .15]{};
	}
      %edges
      \foreach \x in {1,2,...,\nx}{
	\pgfmathsetcount{\xm}{\x-1};
	\draw[edges] (v\x) -- (v\the\xm);
      }
      %draw vertices
      \foreach \x in {0,1,...,\nx}{
        \draw[gray] (\x,0) circle (.9ex); %hack for pdf viewers that do not draw ball shading correctly 
        \shade[ball color=VertexCol] (\x,0) circle (.9ex);% node[beschriftung]{\tiny \x,\y}; 
    % 	\node[fill=white] at (\x,\y) {\tiny \x,\y}; % lable coordinates 
      }
    \end{tikzpicture}
    }
%%% ----------------------- tikz for thermal states ---------------------------------
\newcommand{\drawlattice}{
 \clip (\nx,\ny) ++ (-.5,-.5) rectangle (.5,.5);
  %
  \foreach \x in {0,1,...,\nx}
    \foreach \y in {0,1,...,\ny}
      \node (v\x_\y) [Vertex]  at (\x,\y){}; 
  %edges
  \foreach \x in {1,2,...,\nx}{
    \pgfmathsetcount{\xm}{\x-1};
    \foreach \y in {1,2,...,\ny}{
      \pgfmathsetcount{\ym}{\y-1};
      \draw[edges] (v\x_\y) -- (v\the\xm_\y)
 		  (v\x_\y) -- (v\x_\the\ym);
    }
  }
  %draw vertices
  \foreach \x in {0,1,...,\nx}
    \foreach \y in {0,1,...,\ny}{
      \draw[gray] (\x,\y) circle (\Vsize); %hack for pdf viewers that do not draw ball shading correctly 
      \shade[ball color=VertexCol] (\x,\y) circle (\Vsize);% node[beschriftung]{\tiny \x,\y}; 
% 	\node[fill=white] at (\x,\y) {\tiny \x,\y}; % lable coordinates 
  }
}%

\newcommand{\drawboundary}[5][red]{% #2 \Bx, #3 \By, #4 \Bxsize, #5 \Bysize, #1 color
    \foreach \x in {0, #4}{
      \pgfmathsetcount{\xx}{#2+\x+1};
      \pgfmathsetcount{\xm}{\xx-1};
      \foreach \y in {1,...,#5}{
	\pgfmathsetcount{\yy}{#3+\y};
	\draw[special edges, #1] (v\the\xx_\the\yy) -- (v\the\xm_\the\yy);
      }
    }
    %vertical boundary lines of B
    \foreach \y in {0,#5}{
      \pgfmathsetcount{\yy}{#3+\y+1};
      \pgfmathsetcount{\ym}{\yy-1};
      \foreach \x in {1,...,#4}{
	\pgfmathsetcount{\xx}{#2+\x};
	\draw[special edges, #1] (v\the\xx_\the\yy) -- (v\the\xx_\the\ym);
      }
    }
}

\newcommand{\drawedges}[5][Green]{ % {\Bx}{\By}{\Bxsize}{\Bysize}
      %horizontal lines in B
      \foreach \x in {2,...,#4}{
	\pgfmathsetcount{\xx}{#2 +\x};
	\pgfmathsetcount{\xm}{\xx-1};
	\foreach \y in {1,...,#5}{
	  \pgfmathsetcount{\yy}{#3 +\y};
	  \draw[special edges, #1] (v\the\xx_\the\yy) -- (v\the\xm_\the\yy);
	}
      }
      %vertical lines in B
      \foreach \x in {1,...,#4}{
	\pgfmathsetcount{\xx}{#2 +\x};
	\foreach \y in {2,...,#5}{
	  \pgfmathsetcount{\yy}{#3 +\y};
	  \pgfmathsetcount{\ym}{\yy-1};
	  \draw[special edges, #1] (v\the\xx_\the\yy) -- (v\the\xx_\the\ym);
	}
      }
}

\newcommand{\thermometerBeta}{
    \begin{scope}[scale=2,transform shape, line width=0.4mm, double distance=0.7mm ,
		  xshift=2.65cm, yshift=3.2cm]
    \begin{scope}[rotate=-10]
      \draw[fill=red!90!black] (-0.3,-0.5) circle (0.14);
      \shade[ball color=red!90!black] (-0.3,-0.5) circle (0.14);
      \draw[] (-0.3,-0.5) circle (0.14);
      \draw[double] (-0.3,0.65) -- (-0.3,0);
      \draw[double=red!75!black] (-0.3,0) -- (-0.3,-0.4);
    \end{scope}
    \pgfsetfillopacity{0.85}
    \node[draw,
	  fill=white,
	  name=s,
	  shape=ellipse callout, 
	  callout absolute pointer={(-.1,.1)}, %seems to produce an error
	  inner xsep=0.2cm] 
      at (0.7,0.8) {$1/\beta$};
  \end{scope}  
}

\newcommand{\thermometerBetaR}{
    \begin{scope}[scale=2,transform shape, line width=0.4mm, double distance=0.7mm ,
		  xshift=2.65cm, yshift=3.2cm]
      \begin{scope}[rotate=-10]
	\draw[fill=red!90!black] (-0.3,-0.5) circle (0.14);
	\shade[ball color=red!90!black] (-0.3,-0.5) circle (0.14);
	\draw[] (-0.3,-0.5) circle (0.14);
	\draw[double] (-0.3,0.65) -- (-0.3,0);
	\draw[double=red!75!black] (-0.3,0) -- (-0.3,-0.4);
      \end{scope}
      \pgfsetfillopacity{0.85}
      \node[draw,fill=white,name=s,shape=ellipse callout, callout absolute pointer={(-0.5,.15)},inner 			xsep=0.2cm] at (-1.1,0.8) {$1/\beta$};
    \end{scope}  
}

\newcommand{\thermometerQuestion}{
  \begin{scope}[scale=2,transform shape,line width=0.4mm,double distance=0.7mm, xshift=2.65cm, yshift=3.2cm]
    \begin{scope}[rotate=-10]
      \
      \draw[fill=red!90!black] (-0.3,-0.5) circle (0.14);
      \shade[ball color=red!90!black] (-0.3,-0.5) circle (0.14);
      \draw[] (-0.3,-0.5) circle (0.14);
      \draw[double] (-0.3,0.65) -- (-0.3,-0.2);
      \draw[double=red!75!black] (-0.3,-0.2) -- (-0.3,-0.4) (-0.3,-0.1) -- (-0.3,0) (-0.3,0.1) -- (-0.3,0.3);
    \end{scope}
    \pgfsetfillopacity{0.85}
    \node[draw,fill=white,name=s,shape=cloud callout, aspect=1.5, 
	    callout absolute pointer={(-0.5,0)},
	    inner xsep=0.4cm,inner ysep=0.32cm
	    ] 
	  at (-1.6,0.6)
	  {\begin{tikzpicture}[overlay,xshift=0.05cm,yshift=-0.35cm]
	    \node[use as bounding box] at (0,0.2) {\huge $?$};
	    \node at (0.3,0.3) {\Large $?$};
	    \node at (-0.4,0.4) {\Large $?$};
	    \node at (0,0.6) {$?$};
	    \node at (-0.2,0.1) {$?$};      
	  \end{tikzpicture}
	  };
  \end{scope}
}

\newcommand{\drawSlabel}{
      \path	(\Sx,\Sy) ++(1.5,-1.5) ++(0,\Sysize) 
	node [beschriftung]{$S$};
}

\newcommand{\drawBlabel}{
  \path (\Bx,\By) ++(1.5, -1.5) ++(0,\Bysize)
	    node[beschriftung]{$B$};
}

\newcommand{\drawboundaryBlabel}{
    \path (\Bx,\By) ++(.5,-2.49) ++(0,\Bysize) node[beschriftung, red]{$\I$};
}

\newcommand{\drawAlabel}{\path	(\Sx,\Sy) ++(1.5,-.5) ++(0,\Sysize) node [beschriftung]{$A$};}

\newcommand{\drawdistSB}{
        \draw [|<->|, thick, red!80] (\Bx,\By) ++(.5,3.5) -- ++(2,0) node (mw) [midway]{};
      \path (mw) ++(0,-1.0)  node [beschriftung, red, 
				  inner ysep=.1, inner xsep = .0, 
				  fill = BboxCol, opacity =.7, text opacity = 1]
	    {\small $\dist(S, \I)$};
}


==> tikzset.tex <==
% \colorlet{tensorcol}{niceblue!70!gray}
\colorlet{tensorcol}{NiceGreen!50}
\colorlet{tensorcol}{niceblue!70!gray}
\definecolor{changecol}{rgb}{0.7,0,0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}

\tikzset{
	ol/.style = {remember picture, overlay},
	eq-pic/.style = {inner sep = .5pt,draw, very thick, gray, rounded corners = 2pt},
}

\tikzset{
  connection edge/.style ={very thick, gray},
  generaltensor/.style = {    
    rectangle,
    rounded corners = 0.3mm,
    text = white,
    fill = tensorcol,
    draw
    },
  tensorbox/.style={
    generaltensor,
    inner sep = 2pt, 
    minimum height = 1.1\baselineskip,
    minimum width = 1.1\baselineskip
    },
  tensorleg/.style={
    very thick,black!80
    },
  Vertex/.style={
    % rectangle,minimum size=3mm,rounded corners=1.5mm,
    circle,inner sep=0pt,minimum size=3mm,
%     thick,draw=black!40,
%     top color=white,bottom color=black!20
    },
  site/.style = {
    minimum width = 1.3em, 
    minimum height = 0.5\baselineskip,
    rounded corners=0.3mm,
    thick,draw=black!40,
    top color=white,bottom color=black!20
    },
  channel/.style = {
    generaltensor,
    minimum height=0.5\baselineskip,
    minimum width=1.5cm
  }, 
  ball/.style ={
      circle,
      radius=0.01cm,
      shading=ball, 
      ball color=black}
  }%tikzset
  
\newcount\xm
\newcount\ym
\newcount\xx
\newcount\yy

\pgfdeclarelayer{shadow}
\pgfdeclarelayer{background layer}
\pgfdeclarelayer{foreground layer}
% \pgfsetlayers{shadow,background layer,main, foreground layer} %doesn't work right
\pgfsetlayers{shadow,main}

%%% ----------------------- tikz for thermal states --------------------------------- 
\colorlet{BboxCol}{gray!15}
% \colorlet{SboxCol}{gray!25}
\definecolor{LightYellow}{RGB}{255,255,120}
\colorlet{SboxCol}{LightYellow!80!LightGray}
\colorlet{Green}{OliveGreen}
\colorlet{TextGreen}{OliveGreen!80}
\colorlet{TextBlue}{blue!60}
\colorlet{VertexCol1}{blue!30!LightGray}
\colorlet{VertexCol}{black}
\def \Vsize{1ex}%
\def \nx{6}
\def \ny{6}
\def \Sx{3}
\def \Sy{3}
\def \Sxsize{2}
\def \Sysize{3}  
\def \Bx{1}
\def \By{1}
\def \Bxsize{6}
\def \Bysize{7}
%%% set stuff for own tikzpictures
\tikzset{overlay re oben/.style = {anchor = north east, yshift = -1cm},
	 vertex/.style = {circle,inner sep = 1.2ex},
	 beschriftung/.style = {transform shape = false},
	 box/.style = {rounded corners =.5ex},
	 edges/.style = {thick, line cap = round, gray},
	 special edges/.style = {edges, ultra thick},
	 red edges/.style = {special edges, red!80},
	 green edges/.style = {special edges, Green},
	 lattice/.style = {scale = .54,transform shape, anchor = center}
	 }  

